Coloring Torus Knots by Conjugation Quandles

In the first part of this paper, we present general results concerning the colorability of torus knots using conjugation quandles over any abstract group. Subsequently, we offer a numerical characterization for the colorability of torus knots using conjugation quandles over some particular groups, such as the matrix groups $GL(2,q)$ and $SL(2,q)$, the dihedral group, and the symmetric group.

==> cuts.tex <==
\begin{definition}
    Let $X$ be a nonempty set. We define $\mathsf{T}_Q(X)$, the set of \textbf{quandle terms} on $X$ recursively by
    \begin{enumerate}
        \item $x\in X\implies x\in \mathsf{T}_Q(X)$.
        \item $x,y\in \mathsf{T}_Q(X)\implies x\rhd y\in \mathsf{T}_Q(X)$.
    \end{enumerate}
    The \textbf{free quandle} over $X$ is the quotient algebra $\mathsf{F}_Q(X)=\mathsf{T}_Q(X)/\sim$, where $\sim$ is the congruence generated by the pairs
    $$x\rhd x \sim x,\quad\quad\quad (x\rhd y)\rhd y \sim x, \quad\quad\quad (x\rhd y)\rhd z \sim (x\rhd z)\rhd (y\rhd z).$$
\end{definition}

\begin{definition}
    Let $K$ be a knot (link). The \textbf{fundamental quandle} $\textsf{Q}_K$ of $K$ is the quotient algebra $\mathsf{F}_Q(\arcs(K))/\theta$, where $\theta$ is the congruence generated by all the crossing relations of $K$.
\end{definition}

\begin{theorem}
    The fundamental quandle is a knot (link) full invariant.
\end{theorem}



\begin{theorem} \label{thm:characterization_1}
    Let $m,n\in\N$ be such that $1\le m\le n$ and $\gcd(m,n)=1$, and let $G$ be a group. The following conditions are equivalent:
    \begin{enumerate}
        \item $\K(m,n)$ is $\conj(G)$-colorable.
        \item There are $x_0,\dots,x_{n-1}\in G$ such that all the following terms are equal
        $$\{x_{\sigma^k(0)}x_{\sigma^k(1)}\ldots x_{\sigma^k(m-1)}\colon k=0,\dots,n-1\},$$
        where $\sigma=(0\ 1\ 2\ \dots\ n-1)\in\S_n$ is a cyclic permutation of the indices. \label{thm:char2}
        \item There are $x_0,\dots,x_{n-1}\in G$ such that $$x_i\rhd u = x_{i-m \pmod{n}}\quad\quad\forall i=0,\dots,n-1,$$
    where $u=x_{n-m}x_{n-m+1}\ldots x_{n-2}x_{n-1}$. \label{thm:char3}
    \end{enumerate}
    Moreover, in this case, the element $u$ in \ref{thm:char2} is the common value of the terms in \ref{thm:char3}.
\end{theorem}

\begin{proof} Prove the implications separately. All the indices are assumed to be computed modulo $n$.
    \begin{description}
        \item[$(i)\implies(iii)$] Denote by $x_0,\dots,x_{n-1}$ the colors of horizontal strands, and by $y_0,\dots,y_{m-1}$ the colors of diagonal strands, as in the Figure \ref{fig:k54_xy}. 

        \begin{figure}[h]
            \centering
            \includegraphics[width=.4\linewidth]{pictures/k54_xy.png}
            \caption{Colors in the proof of Theorem \ref{thm:characterization_1}}
            \label{fig:k54_xy}
        \end{figure}
        
        Observe that $x_0=y_0$. By definition of coloring, we have the following relations
        \begin{equation} \label{eqn:yj_train}
            y_j=(((x_j\rhd y_0)\rhd y_1)\rhd\ldots)\rhd y_{j-1}\quad\quad\forall j=0,\dots,m-1.
        \end{equation}
        Moreover, by the geometry of the torus knot, because there are $m$ twists, we also have
        \begin{equation} \label{eqn:xj_train}
            (((x_i\rhd y_0)\rhd y_1)\rhd\ldots)\rhd y_{m-1}=x_{i-m\pmod{n}}\quad\quad\forall i=0,\dots,n-1.
        \end{equation}
        Now, if we expand equations (\ref{eqn:xj_train}), using the quandle axioms and equations (\ref{eqn:yj_train}) and (\ref{eqn:xj_train}) when needed, we obtain
        \begin{align*}
            x_{i-m\pmod{n}}&=(((x_i\rhd y_0)\rhd y_1)\rhd\ldots)\rhd y_{m-1} \\
            &=((((x_i\rhd y_1)\rhd y_2)\rhd\ldots)\rhd y_{m-1})\rhd ((((y_0\rhd y_1)\rhd y_2)\rhd\ldots)\rhd y_{m-1}) \\
            &=((((x_i\rhd y_1)\rhd y_2)\rhd\ldots)\rhd y_{m-1})\rhd x_{n-m} \\
            &=(((((x_i\rhd y_2)\rhd y_3)\rhd\ldots)\rhd y_{m-1})\rhd ((((y_1\rhd y_2)\rhd y_3)\rhd\ldots)\rhd y_{m-1})) \rhd x_{n-m} \\
            &=(((((x_i\rhd y_2)\rhd y_3)\rhd\ldots)\rhd y_{m-1})\rhd x_{n-m+1}) \rhd x_{n-m} \\
            &=\dots \\
            &=(((((x_i\rhd x_{n-1})\rhd x_{n-2})\rhd\ldots)\rhd x_{n-m+2})\rhd x_{n-m+1}) \rhd x_{n-m} \\
            &= (x_{n-m}x_{n-m+1}\ldots x_{n-2}x_{n-1})x_i(x_{n-1}\mo x_{n-2}\mo\ldots x_{n-m+1}\mo x_{n-m}\mo) \\
            &=x_i\rhd u.
        \end{align*}

        \item[$(iii)\implies(i)$] Associate the given elements $x_0,\dots,x_{n-1}$ to the horizontal strands, and compute the colors of diagonal strands $y_0,\dots,y_{m-1}$ recursively as in equations (\ref{eqn:yj_train}). This allows us to compute the color of all other elements in $\arcs(\K(m,n))$ and the conditions $x_i\rhd u = x_{i-m \pmod{n}}$ guarantee the good definition of colors $x_i$'s for the diagram of $\K(m,n)$.
        
        \item[$(ii)\implies(iii)$] Fix $i\in\{0,\dots,n-1\}$. Then, because of $(ii)$, we have 
        \begin{align*}
            x_i\rhd u = ux_iu\mo &= (x_{n-m}x_{n-m+1}\ldots x_{n-2}x_{n-1})x_i(x_{n-m}x_{n-m+1}\ldots x_{n-2}x_{n-1})\mo \\
            &= (x_{n-m+i}x_{n-m+1+i}\ldots x_{n-2+i}x_{n-1+i})x_i(x_{n-m+i+1}x_{n-m+1+i+1}\ldots x_{n-2+i+1}x_{n-1+i+1})\mo \\
            &= (x_{i-m}x_{i-m+1}\ldots x_{i-2}x_{i-1})x_i(x_{i}\mo x_{i-1}\mo \ldots x_{i-m+2}\mo x_{i-m+1}\mo) = x_{i-m}. \\
        \end{align*}

        \item[$(iii)\implies(ii)$] Expand the equations as follows
        \begin{align} \label{eqn:char3_1}
            x_i\rhd u = x_{i-m} \iff (x_{n-m}x_{n-m+1}\ldots x_{n-2}x_{n-1})x_i=x_{i-m}(x_{n-m}x_{n-m+1}\ldots x_{n-2}x_{n-1}).
        \end{align}
        Set $i=0=n$ in (\ref{eqn:char3_1}), and cancel out the term $x_{n-m}$ on the left obtaining
        \begin{align} \label{eqn:char3_2}
            x_{n-m+1}x_{n-m+2}\ldots x_{n-2}x_{n-1}x_i=x_{n-m}x_{n-m+1}\ldots x_{n-2}x_{n-1}
        \end{align}
        which is one of the equations in $(ii)$. Substitute (\ref{eqn:char3_2}) in (\ref{eqn:char3_1}), set $i=n-m+1$, and cancel out the first term again to obtain another equation. Proceeding this way, since $\gcd(m,n)=1$ we obtain the equality of all the terms in $(ii)$.
        
    \end{description}
\end{proof}


\begin{proof}
    Let $x_0,\dots,x_{n-1}$ be a coloring of $\K(m,n)$ and define $$y_j=x_i \iff j\equiv i\pmod{n},\quad\quad\forall j=0,\dots,tn-1.$$
    Because of the conditions $x_i\rhd u =x_{i-m\pmod{n}}$ for $i=0,\dots,n-1$, we also have, for every $j\equiv i\pmod{n}$
    \[
        y_j\rhd u=x_i\rhd u = x_{i-m\pmod{n}} = y_{j-m \pmod{tn}}
    \]
    that is, $y_0,\dots,y_{tn-1}$ is a non-trivial coloring of $\K(m,tn)$.
\end{proof}


The coloring of torus knots has been also studied under another perspective in \cite{Zhou} and \cite{Basi}. In particular, coloring by Alexander Quandles has been completely addressed in \cite{Asami}. We, therefore, proceed with the analysis with conjugation quandles. 

This paper is structured as follows. In Section \ref{sec:fundamentals} we give the preliminary notions regarding torus knots and quandles to be able to introduce what follows. In Section \ref{sec:abstract_groups} we present some general results concerning conjugation quandle colorings of torus knots over any given abstract group, including the main result concerning the characterization of colorability, and some properties of coloring extensions. In the end, in Section \ref{sec:particular_groups} we apply the general results of Section \ref{sec:abstract_groups} in order to achieve characterization theorems for particular groups, such as the matrix groups $\GL(2,q)$ and $\SL(2,q)$, the dihedral
group and the symmetric group. The choice of such particular groups is dual: first of all, they are manageable enough to produce elementary statements for characterization theorem, despite the proofs are rather technical. Moreover, such groups have been studied in other contexts and papers, referred to in the bibliography.


\begin{remark}
    Thanks to Theorem \ref{thm:characterization_1}, with every tuple $(x_0,\dots,x_{n-1})$ of elements of $G$ satisfying the condition in \ref{thm:char3} is associated with a conjugation quandle coloring of $\K(m,n)$, and vice versa. So, when talking about conjugation quandle coloring of a torus knot, we will simply say that the coloring is $(x_0,\dots,x_{n-1})$, implying the validity of the relations \ref{thm:char3}, keeping in mind that we may always construct the full coloring as in the proof of Theorem \ref{thm:characterization_1}. 
\end{remark}



\begin{proposition}
    Let $u\in G$ be a matrix of type 1. Then $\C_G(u)=\C_G(u^p)=G$.
\end{proposition}

\begin{proof}
    The matrix power $u^p$ is still a scalar matrix, hence its centralizer is again maximal.
\end{proof}

\begin{proposition} \label{prop:sl_type2}
    Let $u\in G$ be a matrix of type 2. Then  $\C_G(u^p)\setminus\C_G(u)\neq\emptyset$ if and only if $p\mid q-1$.
\end{proposition}

\begin{proof}
    The matrix power $u^p=\big(\begin{smallmatrix}
    a^p & 0\\
    0 & a^{-p}
    \end{smallmatrix}\big)$ is still diagonal, so its centralizer is strictly larger if and only if $u^p$ is a scalar matrix, that is when $a^p\equiv a^{-p}\pmod{q}$. This happens if and only if $a^{2p}\equiv 1\pmod{q}$ that is when $\mathbb{F}_q^\times$ has an element $a$ of order $2p$. By elementary Group Theory, this is equivalent to the condition $p\mid q-1$.
\end{proof}

\begin{proposition} \label{prop:sl_type3}
    Let $u\in G$ be a matrix of type 3. Then  $\C_G(u^p)\setminus\C_G(u)\neq\emptyset$ if and only if $p=q$.
\end{proposition}

\begin{proof}
    A direct computation shows that the matrix power $$u^p=\begin{pmatrix}
        a & b \\
        0 & a\mo
    \end{pmatrix}^p = 
    \begin{pmatrix}
        a^p & b\sum_{k=0}^{p-1}a^{2k+1-p} \\
        0 & a^{-p}
    \end{pmatrix} = 
    \begin{pmatrix}
        a & b\sum_{k=0}^{p-1}a^{2k+1-p} \\
        0 & a\mo
    \end{pmatrix}$$
    has the same centralizer as the matrix $u$, unless $b\sum_{k=0}^{p-1}a^{2k+1-p}\equiv 0\pmod{q}$. Being $a^2=1$ and $b\neq 0$, this happens if and only if $p=q$.
\end{proof}

\begin{proposition} \label{prop:sl_type4}
    Let $u\in G$ be a matrix of type 4. Then  $\C_G(u^p)\setminus\C_G(u)\neq\emptyset$ if and only if $p\mid q+1$.
\end{proposition}

\begin{proof}
    It is a special case of the proof given for $\GL(2,q)$.
\end{proof}

Additionally, based on Remark \ref{rmk:kmn_equals_knm}, when studying $\K(m,p)$ for $p$ prime, we may always assume that $p\neq 2$. Indeed, if $p$ was 2, our assumptions $m\le 2$ and $\gcd(m,2)=1$ would force $m=1$. However, $\K(1,2)$ is the trivial knot, which is only trivially colorable. Consequently, when studying $\K(m,p)$ we can always assume that $m\ge 2$ and $p\ge 3$ is prime such that $p\nmid m$.
